Data-Driven Fast Frequency Control using Inverter-Based Resources

To address the control challenges associated with the increasing share of inverter-connected renewable energy resources, this paper proposes a direct data-driven approach for fast frequency control in the bulk power system. The proposed control scheme partitions the power system into control areas, and leverages local dispatchable inverter-based resources to rapidly mitigate local power imbalances upon events. The controller design is based directly on historical measurement sequences, and does not require identification of a parametric power system model. Theoretical results are provided to support the approach. Simulation studies on a nonlinear three-area test system demonstrate that the controller provides fast and localized frequency control under several types of contingencies.

==> confpaperdefs.tex <==
% -------- Packages ---------
\usepackage{etex}
\usepackage[vlined,ruled]{algorithm2e}
\usepackage[dvipsnames]{xcolor}
\usepackage{pgfpages}
\usepackage[cmex10]{amsmath}		%Load Fonts
\usepackage{amssymb, mathrsfs}
\usepackage{cite}
\usepackage{url}

% Computer Modern Font
%\usepackage{lmodern}						%Load Modern Font
%\usepackage[T1]{fontenc}					%T1-Font Encoding
%\renewcommand*\familydefault{\sfdefault}	%Sans-Serif Base Font

\usepackage{dsfont}
\usepackage{siunitx}
\usepackage{verbatim}									%verbatim and comment environemtns		
\usepackage{mathtools}									%used for xmapsto command
\usepackage{siunitx}									%load SI units
\usepackage{mdframed}

\usepackage{graphicx}
\usepackage{epstopdf}

\usepackage[font=small]{caption}
\usepackage{subcaption}
\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}

\usepackage{array}
\usepackage{multirow}
\usepackage{enumerate}
\usepackage{booktabs}

% ----

\graphicspath{{./fig/}}



%-------------------------------
%-------- PGF-Plots ------------
%-------------------------------

\newcommand*{\strongconvex}{2}
\newcommand*{\feedforward}{0.9}


%http://pgfplots.sourceforge.net/gallery.html

\usepackage{pgfplots}
\pgfplotsset{width=8cm,compat=newest}
\newcommand*{\damping}{0.006}%
\newcommand*{\freq}{25}%
\pgfmathsetmacro{\freqd}{sqrt(1-(\damping)^2)*\freq}%

\pgfplotsset{
    standard/.style={
    axis x line=middle,
    axis y line=middle,
    enlarge x limits=0.15,
	enlarge y limits=0.15,
	%every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
	%every axis y label/.style={at={(current axis.above origin)},anchor=north east},
	%x label/.style={at={(axis description cs:1.05,0.16)},anchor=north},
	%y label/.style={at={(axis description cs:0.2,1.05)},anchor=north},
	every axis plot post/.style={mark options={fill=black}},
	%every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
    %every axis y label/.style={at={(current axis.above origin)},anchor=north east}
	}
}

\pgfplotsset{%
    ,compat=1.12
    ,every axis x label/.style={at={(current axis.right of origin)},anchor=north west}
    ,every axis y label/.style={at={(current axis.above origin)},anchor=north east}
    }



%-------------------------
%--------- Tikz ----------
%-------------------------

\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{snakes}
\usetikzlibrary{matrix}
\usetikzlibrary{calc}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes.callouts}
\usetikzlibrary{shapes.misc}

\tikzstyle{every node}=[font=\small]
\tikzstyle{every path}=[line width=0.8pt,line cap=round,line join=round]
\newcommand{\midarrow}{\tikz \draw[-triangle 90] (0,0) -- +(.1,0);}


%------- Circuit Tikz ----------
\usepackage[american,smartlabels]{circuitikz}
\ctikzset{bipoles/thickness=1}
\ctikzset{bipoles/length=0.8cm}
\ctikzset{bipoles/diode/height=.375}
\ctikzset{bipoles/diode/width=.3}
\ctikzset{tripoles/thyristor/height=.8}
\ctikzset{tripoles/thyristor/width=1}
\ctikzset{bipoles/vsourceam/height/.initial=.7}
\ctikzset{bipoles/vsourceam/width/.initial=.7}


%------ My commands ---------
\newcommand{\real}{\mathbb{R}}
\newcommand{\mymod}[1]{\textup{mod}#1}
\newcommand{\realnonnegative}{\mathbb{R}_{\geq0}}
\newcommand{\until}[1]{\{1,\dots, #1\}}												
\newcommand{\complex}{\mathbb{C}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\disk}{\mathbb{D}}
\newcommand{\mycircle}{\ensuremath{\mathbb S^{1}}}
\newcommand{\sphere}{\ensuremath{\mathbb S}}
\newcommand{\torus}{\ensuremath{\mathbb T}}
\newcommand{\setdef}[2]{\{#1 \;|\; #2\}}
\newcommand{\bigsetdef}[2]{\big\{#1 \; | \; #2\big\}}
\newcommand{\union}{\operatorname{\cup}}
\newcommand{\intersection}{\ensuremath{\operatorname{\cap}}}
\newcommand{\arc}{\textup{Arc}_{n}}
\newcommand{\bararc}{\overline{\mbox{Arc}}_{n}}
\newcommand{\PQ}{\textsf{PQ} }
\newcommand{\PV}{\textsf{PV} }
\newcommand{\mytt}[1]{\textup{\texttt{#1}}\xspace}
\renewcommand{\j}{\boldsymbol{\mathrm{j}}}
\renewcommand{\arc}{\operatorname{Arc}_{n}}
\newcommand{\abs}[1]{\left\lvert{#1}\right\rvert}                     			% \abs{x} -->  |x| with proper spacing
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}                     		% \norm{x} -->  ||x|| with proper spacing
\DeclareMathOperator*{\minimize}{minimize} 									% minimize
\DeclareMathOperator*{\maximize}{maximize} 									% maximize
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\sinc}{sinc}
\DeclareMathOperator*{\sinbf}{\mathrm{\bf sin}} 	                              %
\DeclareMathOperator*{\cosbf}{\mathrm{\bf cos}} 	                              %
\DeclareMathOperator*{\sincbf}{\mathrm{\bf sinc}} 	                              %
\DeclareMathOperator*{\arcsinbf}{\mathrm{\bf arcsin}} 	
\newcommand{\bsin}{\boldsymbol{\sin}}
\newcommand{\barcsin}{\boldsymbol{\arcsin}}
\newcommand{\bcos}{\boldsymbol{\cos}}
\newcommand{\bln}{\boldsymbol{\mathrm{ln}}}
                              

\newcommand{\vect}[1]{\mathbbold{#1}}
\newcommand{\vones}[1][]{\vect{1}_{#1}}
\newcommand{\vzeros}[1][]{\vect{0}_{#1}}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}

\newcommand{\map}[3]{#1: #2 \rightarrow #3}

\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\deg}{\mathrm{deg}}

\renewcommand{\theenumi}{(\roman{enumi})}
\renewcommand{\labelenumi}{\theenumi}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\tr}{\color{red}}
\newcommand{\tv}{\color{violet}}
\newcommand{\tb}{\color{blue}}
\newcommand{\john}[1]{{\leavevmode\color{blue}\textbf{From John:\;}#1}}
\newcommand{\johnref}{\textbf{\textcolor{red}{[ref] }}}
\newcommand\fyimargin[1]{\marginpar{\color{violet} \small\ttfamily FYI (read and erase): #1}}
\newcommand{\todo}[1]{\par\noindent{\color{blue}\raggedright\textsc{#1}\par\marginpar{\large$\star$}}}
\newcommand{\fdmargin}[1]{\marginpar{\color{blue}\tiny\ttfamily{FD:} #1}}
\newcommand{\jsmargin}[1]{\marginpar{\color{red}\tiny\ttfamily{JS:} #1}}
\newcommand{\fbmargin}[1]{\marginpar{\color{red}\small\ttfamily{FB:} #1}}
\newcommand{\bpmargin}[1]{\marginpar{\bf \color{violet}\tiny\ttfamily{BP:} #1}}
\newcommand{\nmargin}[1]{\marginpar{\color{blue}\tiny\ttfamily{NM:} #1}}


% custom made commands
\newcommand*\fvec[1]{\ensuremath{\mathbf{#1}}}                           % creates a bold symbol
\newcommand{\transpose}{\mathsf{T}} %or \top or \intercal				% transpose symbol


% Procend
\newcommand\oprocendsymbol{\hbox{$\square$}}
\newcommand\oprocend{\relax\ifmmode\else\unskip\hfill\fi\oprocendsymbol}
\def\eqoprocend{\tag*{$\square$}}

%Theorem Environments

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}

\newenvironment{pfof}[1]{\vspace{1ex}\noindent{\itshape Proof of
    #1:}\hspace{0.5em}} {\hfill\oprocend\vspace{1ex}}

% -------------------------------------
% ---------- Boyd Commands ------------
% -------------------------------------

\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\prox}{\mathbf{prox}}

\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\epi}{\mathop{\bf epi}} % epigraph
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} % domain
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\sign}{\mathop{\bf sign}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}
\newcommand{\define}{\coloneqq}




%-----------------------------------------------------
%-------- Conditional Statements and Hiding -----------
%-----------------------------------------------------

\newif\ifforstudents

\newcommand{\hide}[1]{
    \ifforstudents{
        \leavevmode\hphantom{#1}
    }
    \else{
        #1
    }
    \fi
}


\newcommand{\hideq}[1]{
    \ifforstudents{
        \boxed{\phantom{#1}}
    }
    \else{
        #1
    }
    \fi
}


\newcommand{\hideqnobox}[1]{
    \ifforstudents{
        \phantom{#1}
    }
    \else{
        #1
    }
    \fi
}


\newcommand{\hidetikz}[1]{
    \ifforstudents{
    	\tikzset{every picture/.append style={
				 execute at end picture={
				\fill [white] ([yshift=-0.2cm]current bounding box.south west) rectangle ([yshift=0.1cm]current bounding box.north east);
}}}#1
    }
    \else{
        #1
    }
    \fi
}




